Piecewise Robust Barrier Tubes for Nonlinear Hybrid Systems with Uncertainty

Piecewise Barrier Tubes (PBT) is a new technique for flowpipe overapproximation for nonlinear systems with polynomial dynamics, which leverages a combination of barrier certificates. PBT has advantages over traditional time-step based methods in dealing with those nonlinear dynamical systems in which there is a large difference in speed between trajectories, producing an overapproximation that is time independent. However, the existing approach for PBT is not efficient due to the application of interval methods for enclosure-box computation, and it can only deal with continuous dynamical systems without uncertainty. In this paper, we extend the approach with the ability to handle both continuous and hybrid dynamical systems with uncertainty that can reside in parameters and/or noise. We also improve the efficiency of the method significantly, by avoiding the use of interval-based methods for the enclosure-box computation without loosing soundness. We have developed a C++ prototype implementing the proposed approach and we evaluate it on several benchmarks. The experiments show that our approach is more efficient and precise than other methods in the literature.

==> include/RBT4HybridSystem.tex <==
\section{Robust Barrier Tubes for Hybrid Systems}

==> include/acknowledgement.tex <==
\section*{Acknowledgment}
This research was supported in part by the Austrian Science Fund (FWF)
under grants S11402-N23, S11405-N23 (RiSE/SHiNE) and Z211-N23 (Wittgenstein
Award).

==> include/relatedwork.tex <==
\section{Related Work}\label{sec:relatedwork}

Many recent efforts have been made toward generating invariants for hybrid systems. Matringe et al.\ reduce the invariant generation problem to the computation of the associated eigenspaces by encoding the invariant constraints as symbolic matrices~\cite{rebiha2015generating}. Ghorbal et al.\ use the invariant algebraic set formed by a polynomial and a finite set of its successive Lie derivatives to overapproximate vector flows~\cite{ghorbal2014characterizing}. Both of the aforementioned methods involve minimizing the rank of a symbolic matrix. Although in theory the problem of minimizing the rank of a symbolic matrix lies in the same complexity class as that of our problem, experiments show that our approach is more powerful in practice. Sankaranarayanan discovers invariants based on invariant ideal and pseudo ideal iteration~\cite{sankaranarayanan2010automatic}, but this method is limited to algebraic systems. Moreover, none of the aforementioned methods involve verifying safety properties based on the invariants obtained. Tiwari et al.\ compute invariants for some special types of linear and nonlinear systems based on \emph{Syzygy} computation and \Groba theory as well as linear constraint solving~\cite{tiwari2004nonlinear}. Platzer et al.\ use quantifier elimination to find differential invariants~\cite{platzer2008computing}. Another approach considers barrier certificates based on different inductive conditions~\cite{prajna2004safety,kong2013exponential,kong2014new} which can be solved by \SOS programming efficiently but is limited by the conservative inductive condition. Carbonell et al.\ generate invariants for linear systems~\cite{rodriguez2005generating}. Some other approaches focusing on different features of systems have also been proposed for constructing inductive invariants~\cite{johnson2013invariant,gulwani2008constraint,
  sankaranarayanan2004constructing,sassi2014iterative,liu2011computing,
  goubault2014finding}. 

